Stereographic Markov Chain Monte Carlo

High-dimensional distributions, especially those with heavy tails, are notoriously difficult for off-the-shelf MCMC samplers: the combination of unbounded state spaces, diminishing gradient information, and local moves results in empirically observed ``stickiness'' and poor theoretical mixing properties -- lack of geometric ergodicity. In this paper, we introduce a new class of MCMC samplers that map the original high-dimensional problem in Euclidean space onto a sphere and remedy these notorious mixing problems. In particular, we develop random-walk Metropolis type algorithms as well as versions of the Bouncy Particle Sampler that are uniformly ergodic for a large class of light and heavy-tailed distributions and also empirically exhibit rapid convergence in high dimensions. In the best scenario, the proposed samplers can enjoy the ``blessings of dimensionality'' that the convergence is faster in higher dimensions.

==> Sec-Ergodicity.tex <==
	\section{PDMP on Sphere: Uniform Ergodicity}
	\label{sec-PDMP-UE}


==> commenting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% EDITING HELPER FUNCTIONS  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% NA: needs attention (rough writing whose correctness needs to be verified)
%% TBD: instructions for how to fix a gap ("Describe the propagation by ...")
%% PROBLEM: bug or missing crucial bit 

%% use \fXXX versions of these macros to put additional explanation into a footnote.  
%% The idea is that we don't want to interrupt the flow of the paper or make it 
%% impossible to read because there are a bunch of comments.

%% NA's (and TBDs, those less crucially) should be written so 
%% that they flow with the text.

\definecolor{WowColor}{rgb}{.75,0,.75}
\definecolor{SubtleColor}{rgb}{0,0,.50}

% inline
\newcommand{\RED}[1]{\textcolor{red}{#1}}
\newcommand{\NA}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\star$)} #1}}
\newcommand{\LATER}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\dagger$)} #1}}
\newcommand{\TBD}[1]{\textcolor{SubtleColor}{ {\tiny \bf (!)} #1}}
\newcommand{\PROBLEM}[1]{\textcolor{WowColor}{ {\bf (!!)} {\bf #1}}}

% as margin notes

\newcounter{margincounter}
\newcommand{\displaycounter}{{\arabic{margincounter}}}
\newcommand{\incdisplaycounter}{{\stepcounter{margincounter}\arabic{margincounter}}}

\newcommand{\fTBD}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter)$} #1}}}

\newcommand{\fPROBLEM}[1]{\textcolor{WowColor}{$\,^{((\incdisplaycounter))}$}\marginpar{\tiny\textcolor{WowColor}{ {\bf $\mathbf{((\displaycounter))}$} {\bf #1}}}}

\newcommand{\fLATER}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter\dagger)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter\dagger)$} #1}}}


==> defs.tex <==
% !TEX root =  paper.tex

\def\[#1\]{\begin{align}#1\end{align}}
\def\*[#1\]{\begin{align*}#1\end{align*}}

\newcommand{\lati}{y_{d+1}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\ZO}{\mathbb B} %by JY
\newcommand{\normal}{\mathcal N}
%\newcommand{\trace}{\textrm{tr}}
\DeclareMathOperator*{\trace}{tr}	 
\DeclareMathOperator*{\PG}{PG}	 
\DeclareMathOperator*{\SP}{SP}
\DeclareMathOperator*{\GSP}{GSP}	
\DeclareMathOperator*{\diag}{Diag}	
\newcommand{\defas}{\vcentcolon=}  % requires mathtools package
%\newcommand{\defas}{\equiv}

%% such that
\newcommand{\st}{\,:\,}

%% for writing  A | X ~ P(X) statements
\newcommand{\dist}{\ \sim\ }
\newcommand{\given}{\mid}
\newcommand{\distiid}{\overset{iid}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}


\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\BorelSets}{\mathcal{B}}
\newcommand{\Nats}{\mathbb{N}}
\newcommand{\Ints}{\mathbb{Z}}
\newcommand{\NNInts}{\Ints_+}
\newcommand{\NNExtInts}{\overline{\Ints}_+}
\newcommand{\Cantor}{\2^\mathbb{N}}
\newcommand{\NNReals}{\Reals_+}

\newcommand{\as}{\textrm{a.s.}}

\newcommand{\epi}{\textrm{epi}}
\newcommand{\intr}{\textrm{int}}
\newcommand{\conv}{\textrm{conv}}
\newcommand{\cone}{\textrm{cone}}
\newcommand{\aff}{\textrm{aff}}
\newcommand{\dom}{\textrm{dom}}
\newcommand{\cl}{\textrm{cl}}
\newcommand{\ri}{\textrm{ri}}
\newcommand{\grad}{\nabla}
\newcommand{\imp}{\Rightarrow}
\newcommand{\downto}{\!\downarrow\!}
\newcommand{\upto}{\!\uparrow\!}

%\newcommand{\ind}{\perp\!\!\!\perp}
\newcommand{\ind}{\mathrel{\perp\mkern-9mu\perp}}
%\newcommand\ind{\protect\mathpalette{\protect\independenT}{\perp}} 
%\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern5mu{#1#2}}}

\newcommand{\AND}{\wedge}
\newcommand{\OR}{\vee}
\newcommand{\NOT}{\neg}

\newcommand{\dee}{\mathrm{d}}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\ESJD}{ESJD}

\DeclareMathOperator*{\newlim}{\mathrm{lim}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newmin}{\mathrm{min}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newmax}{\mathrm{max}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newinf}{\mathrm{inf}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newsup}{\mathrm{sup}\vphantom{\mathrm{infsup}}}
\renewcommand{\lim}{\newlim}
\renewcommand{\min}{\newmin}
\renewcommand{\max}{\newmax}
\renewcommand{\inf}{\newinf}
\renewcommand{\sup}{\newsup}

%\newcommand{\card}[1]{\#(#1)}
\newcommand{\PowerSet}{\mathcal{P}}

\newcommand{\Measures}{\mathcal{M}}
\newcommand{\ProbMeasures}{\mathcal{M}_1}

\renewcommand{\Pr}{\mathbb{P}}
\def\EE{\mathbb{E}}
\DeclareMathOperator*{\var}{var}

%% definition 
\newcommand{\defn}[1]{\emph{#1}}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceiling}[1]{\lceil #1 \rceil}

\def\bone{\mathbf{1}}
\def\Ind{\bone}

\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}

\DeclareMathOperator*{\Beta}{Beta}
\DeclareMathOperator*{\Bernoull}{Bernoulli}
\DeclareMathOperator*{\PP}{PP}
\DeclareMathOperator*{\Poisson}{Poisson}
\newcommand{\Uniform}{\textrm U (0,1)}

\newcommand{\equaldist}{\overset{d}{=}}
\newcommand{\inv}{^{-1}}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\event}[1]{\left \lbrace #1 \right \rbrace}
\newcommand{\tuple}[1]{\langle #1 \rangle}


\newcommand{\bspace}{\Omega}
\newcommand{\bsa}{\mathcal A}
\newcommand{\borelspace}{(\bspace,\bsa)}


\newcommand{\card}[1]{\##1}
%\newcommand{\as}{\textrm{a.s.}}
\newcommand{\iid}{i.i.d.}

%% for writing down stochastic processes
\newcommand{\gprocess}[2]{(#1)_{#2}}
\newcommand{\nprocess}[3]{\gprocess{#1_{#3}}{#3 \in #2}}
\newcommand{\process}[2]{\nprocess{#1}{#2}n}


%% not in love with these...
\newcommand{\of}[1]{\left ( #1 \right )}
\newcommand{\oof}[1]{( #1 )}
\newcommand{\ooof}[1]{\bigl ( #1 \bigr )}
\newcommand{\oooof}[1]{\Bigl ( #1 \Bigr )}
\newcommand{\ooooof}[1]{\biggl ( #1 \biggr )}
\newcommand{\oooooof}[1]{\Biggl ( #1 \Biggr )}

\newcommand{\oF}[1]{\left [ #1 \right ]}
\newcommand{\ooF}[1]{[ #1 ]}
\newcommand{\oooF}[1]{\bigl [ #1 \bigr ]}
\newcommand{\ooooF}[1]{\Bigl [ #1 \Bigr ]}
\newcommand{\oooooF}[1]{\biggl [ #1 \biggr ]}
\newcommand{\ooooooF}[1]{\Biggl [ #1 \Biggr ]}

\newcommand{\Of}[1]{\left \{ #1 \right \}}
\newcommand{\Oof}[1]{\{ #1 \}}
\newcommand{\Ooof}[1]{\bigl \{ #1 \bigr \}}
\newcommand{\Oooof}[1]{\Bigl \{ #1 \Bigr \}}
\newcommand{\Ooooof}[1]{\biggl \{ #1 \biggr \}}
\newcommand{\Oooooof}[1]{\Biggl \{ #1 \Biggr \}}


%% added by Jun Yang
\newcommand{\TMarginal}{\Truth^1}
\newcommand{\TPosterior}{\Truth^2}
%\newcommand{\AND}{\wedge}
%\newcommand{\OR}{\vee}
%\newcommand{\NOT}{\neg}

%\newcommand{\dee}{\mathrm{d}}

%\newcommand{\ProbMeasures}{\mathcal{M}_1}
%\newcommand{\defas}{\vcentcolon=}
\renewcommand{\appendixname}{}
%\renewcommand{\sectionname}{\S}
%\newcommand{\NNReals}{\Reals_+}
%\newcommand{\Reals}{\mathbb{R}}
\newtheorem{assumption}{Assumption}
\newtheorem*{assumption*}{Assumption}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\newcommand{\KL}[2]{\mathrm{KL}\left(#1 || #2\right)}
%%\newcommand{\conv}{\textrm{conv}}
%%\newcommand{\defn}[1]{\emph{#1}}

\newcommand{\XX}{\mathcal X}
\newcommand{\YY}{\mathcal Y}
\newcommand{\Actions}{\mathcal A}
\newcommand{\Algorithms}{\mathcal F}
\newcommand{\Model}{Q}
\newcommand{\Truth}{P}
\newcommand{\prior}{\pi}
\newcommand{\optset}{\Pi}
%\newcommand{\Nats}{\mathbb{N}}

\newcommand{\disint}[3]{(#1#2|#3)}


==> headers-aos.tex <==
% !TEX root = draft_metabayes.tex

%\usepackage{amsaddr}
%\usepackage[foot]{amsaddr}
\usepackage[utf8]{inputenc} 
\usepackage{amsmath, amssymb,bm, cases, mathtools, thmtools, bbm}
\usepackage{verbatim}
\usepackage{graphicx}\graphicspath{{figures/}}
\usepackage{multicol}
\usepackage{tabularx}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{mathrsfs} 
\usepackage{url}

\usepackage{biblatex}
%\usepackage[%
 %   minnames=4,maxnames=99,maxcitenames=4,
  %  style=alphabetic,
  %  doi=false,url=false,
  %  firstinits=true,hyperref,natbib,backend=bibtex]{biblatex}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
%\bibliography{biblio}
\bibliography{mcmc2} %changed by Jun Yang

\usepackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=RawSienna]{hyperref}
\usepackage{hypernat}
\usepackage{datetime}

%% change up the fonts for fun.
%\usepackage[OT1]{eulervm} 
%\usepackage{palatino}

\DeclareMathAlphabet\EuRoman{U}{eur}{m}{n}
\SetMathAlphabet\EuRoman{bold}{U}{eur}{b}{n}
\newcommand{\eurom}{\EuRoman}

%% hide equation numbers for unreferenced equations
%\mathtoolsset{showonlyrefs}

%% make text prettier
\usepackage{euscript,microtype}
%\DisableLigatures{encoding = *, family = * }

%% nicer way of making \ref'ences to theorems, lemmas, equations, sections, etc.
\usepackage[capitalize]{cleveref}

%% add entries for anything missing.
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{theorem}{Theorem}{Theorems}

%% grey out the equation numbers slightly
\makeatletter
\let\reftagform@=\tagform@
\def\tagform@#1{\maketag@@@{\ignorespaces\textcolor{gray}{(#1)}\unskip\@@italiccorr}}
\renewcommand{\eqref}[1]{\textup{\reftagform@{\ref{#1}}}}
\makeatother


%% standard marginalia note
\setlength{\marginparwidth}{1.25in}

%% reshape the page to make it wider
%\usepackage[paperwidth=185.7mm,
%      paperheight=241.2mm,
%      textwidth=140mm,
%      textheight=230mm,
%      left=12mm]{geometry}
%\setlength{\marginparwidth}{27mm}

%% Monitor
%\usepackage[paperwidth=8in,paperheight=9in,textwidth=6in, textheight=8in,left=.5in]{geometry}
%\setlength{\marginparwidth}{1.5in}

\input{commenting.tex}

%% For submission, make all render blank.
%\renewcommand{\LATER}[1]{}
%\renewcommand{\fLATER}[1]{}
%\renewcommand{\TBD}[1]{}
%\renewcommand{\fTBD}[1]{}
%\renewcommand{\PROBLEM}[1]{}
%\renewcommand{\fPROBLEM}[1]{}
%\renewcommand{\NA}[1]{#1}  %% Note, NA's pass through!


%% theorem styles
\declaretheorem[style=plain,numberwithin=section,name=Theorem]{theorem}
\declaretheorem[style=plain,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=plain,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=plain,sibling=theorem,name=Corollary]{corollary}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,sibling=theorem,name=Example]{example}
\declaretheorem[style=remark,sibling=theorem,name=Remark]{remark}
\declaretheorem[style=definition,sibling=theorem]{fact}

%\numberwithin{equation}{section}
\numberwithin{theorem}{section}

\renewcommand{\appendixname}{}
%\renewcommand{\sectionname}{\S}

%% put ruler down the side for draft, and color it gray
%\usepackage{vruler}
%\setvruler[10pt][1][1][4][1][20pt][20pt][0pt][\textheight]
%\let\orgfillzeros\fillzeros 
%\def\fillzeros[#1]#2{% 
%  \begingroup 
%    \color[rgb]{0.8,0.8,0.8}% 
%    \orgfillzeros[{#1}]{#2}% 
%  \endgroup 
%}


==> headers.tex <==
% !TEX root = draft_metabayes.tex

%\usepackage{amsaddr}
\usepackage[foot]{amsaddr}
\usepackage[utf8]{inputenc} 
\usepackage{amsmath, amssymb,bm, cases, mathtools, thmtools, bbm}
\usepackage{verbatim}
\usepackage{graphicx}\graphicspath{{figures/}}
\usepackage{multicol}
\usepackage{tabularx}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{mathrsfs} 
\usepackage{url}

\usepackage[%
    minnames=4,maxnames=99,maxcitenames=4,
    style=alphabetic,
    doi=false,url=false,
    firstinits=true,hyperref,natbib,backend=bibtex]{biblatex}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
%\bibliography{biblio}
\bibliography{mcmc2} %changed by Jun Yang

\usepackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=RawSienna]{hyperref}
\usepackage{hypernat}
\usepackage{datetime}

%% change up the fonts for fun.
%\usepackage[OT1]{eulervm} 
%\usepackage{palatino}

\DeclareMathAlphabet\EuRoman{U}{eur}{m}{n}
\SetMathAlphabet\EuRoman{bold}{U}{eur}{b}{n}
\newcommand{\eurom}{\EuRoman}

%% hide equation numbers for unreferenced equations
%\mathtoolsset{showonlyrefs}

%% make text prettier
\usepackage{euscript,microtype}
%\DisableLigatures{encoding = *, family = * }

%% nicer way of making \ref'ences to theorems, lemmas, equations, sections, etc.
\usepackage[capitalize]{cleveref}

%% add entries for anything missing.
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{theorem}{Theorem}{Theorems}

%% grey out the equation numbers slightly
\makeatletter
\let\reftagform@=\tagform@
\def\tagform@#1{\maketag@@@{\ignorespaces\textcolor{gray}{(#1)}\unskip\@@italiccorr}}
\renewcommand{\eqref}[1]{\textup{\reftagform@{\ref{#1}}}}
\makeatother


%% standard marginalia note
\setlength{\marginparwidth}{1.25in}

%% reshape the page to make it wider
%\usepackage[paperwidth=185.7mm,
%      paperheight=241.2mm,
%      textwidth=140mm,
%      textheight=230mm,
%      left=12mm]{geometry}
%\setlength{\marginparwidth}{27mm}

%% Monitor
%\usepackage[paperwidth=8in,paperheight=9in,textwidth=6in, textheight=8in,left=.5in]{geometry}
%\setlength{\marginparwidth}{1.5in}

\input{commenting.tex}

%% For submission, make all render blank.
%\renewcommand{\LATER}[1]{}
%\renewcommand{\fLATER}[1]{}
%\renewcommand{\TBD}[1]{}
%\renewcommand{\fTBD}[1]{}
%\renewcommand{\PROBLEM}[1]{}
%\renewcommand{\fPROBLEM}[1]{}
%\renewcommand{\NA}[1]{#1}  %% Note, NA's pass through!


%% theorem styles
\declaretheorem[style=plain,numberwithin=section,name=Theorem]{theorem}
\declaretheorem[style=plain,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=plain,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=plain,sibling=theorem,name=Corollary]{corollary}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem,name=Example]{example}
\declaretheorem[style=remark,qed=$\triangleleft$,sibling=theorem,name=Remark]{remark}
%\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem]{fact}

%\numberwithin{equation}{section}
\numberwithin{theorem}{section}

\renewcommand{\appendixname}{}
%\renewcommand{\sectionname}{\S}

%% put ruler down the side for draft, and color it gray
%\usepackage{vruler}
%\setvruler[10pt][1][1][4][1][20pt][20pt][0pt][\textheight]
%\let\orgfillzeros\fillzeros 
%\def\fillzeros[#1]#2{% 
%  \begingroup 
%    \color[rgb]{0.8,0.8,0.8}% 
%    \orgfillzeros[{#1}]{#2}% 
%  \endgroup 
%}

